Presupernova evolution and explosive nucleosynthesis of rotating massive stars in the metallicity range -3 <=[Fe/H]<= 0

We present a new grid of presupernova models of massive stars extending in mass between 13 and 120 Msun, covering four metallicities (i.e. [Fe/H]=0, -1, -2 and -3) and three initial rotation velocities (i.e. 0, 150 and 300 km/s). The explosion has been simulated following three different assumptions in order to show how the yields depend on the remnant mass - initial mass relation. An extended network from H to Bi is fully coupled to the physical evolution of the models. The main results can be summarized as follows. a) At solar metallicity the maximum mass exploding as Red Super Giant (RSG) is of the order of 17 Msun in the non rotating case, all the more massive stars exploding as WR stars. All rotating models, vice versa, explode as Wolf-Rayet (WR) stars. b) The interplay between the core He burning and the H burning shell, triggered by the rotation induced instabilities, drives the synthesis of a large primary amount of all the products of the CNO, not just N14. A fraction of them enriches enormously the radiative part of the He core (and is responsible of the large production of F) and a fraction enters the convective core leading therefore to an important primary neutron flux able to synthesize heavy nuclei up to Pb. c) In our scenario, remnant masses of the order of those inferred by the first detections of the gravitational waves (GW150914, GW151226, GW170104, GW170814) are predicted at all metallicities for none or moderate initial rotation velocities.

==> tab_special_reactions.tex <==
\floattable                              
\startlongtable
\begin{deluxetable*}{ccccccccccccccc}
\tablecolumns{2}
\tabletypesize{\scriptsize}
%\tablewidth{0pt}
\tablecaption{Network reference matrix for special nuclear reactions \label{crosspecial}}
\tablehead{
\colhead{reaction} &
\colhead{($\beta^+$)} & \colhead{reference} }
\startdata   
         p             (p            ,$\rm e^+\nu$)$\rm ^{2}H$   & nacr    \\
         $\rm ^{3}He$  ($\rm ^{3}He$ ,2p          )$\rm \alpha$  & nacr    \\
         $\rm \alpha$  ($\rm ^{3}He$ ,$\rm \gamma$)$\rm ^{7}Be$  & cy08    \\
         $\rm ^{2}H$   ($\rm ^{2}H$  ,p           )$\rm ^{3}H$   & nacr    \\       
         $\rm ^{2}H$   ($\rm ^{2}H$  ,n           )$\rm ^{3}He$  & desc    \\                  
         $\rm ^{2}H$   ($\rm ^{2}H$  ,$\rm \gamma$)$\rm \alpha$  & nacr    \\
         $\rm ^{3}H$   (p            ,$\rm ^{2}H$ )$\rm ^{2}H$   & nacr    \\       
         $\rm ^{3}H$   ($\rm ^{2}H$  ,n           )$\rm \alpha$  & desc    \\       
         $\rm ^{3}He$  ($\rm ^{2}H$  ,p           )$\rm \alpha$  & desc    \\       
         $\rm ^{3}He$  ($\rm ^{3}H$  ,$\rm ^{2}H$ )$\rm \alpha$  & cf88    \\       
         $\rm ^{3}He$  (n            ,$\rm ^{2}H$ )$\rm ^{2}H$   & desc    \\                  
         $\rm 2\alpha$ ($\rm \alpha$ ,$\rm \gamma$)$\rm ^{12}C$  & nacr    \\
         $\rm \alpha$  (p            ,$\rm ^{2}H$ )$\rm ^{3}He$  & desc    \\
         $\rm \alpha$  ($\rm ^{2}H$  ,$\rm ^{3}H$ )$\rm ^{3}He$  & cf88    \\
         $\rm \alpha$  ($\rm ^{3}H$  ,n           )$\rm ^{6}Li$  & cf88    \\
         $\rm \alpha$  ($\rm ^{3}H$  ,n           )$\rm ^{6}Li$  & desc    \\
         $\rm \alpha$  ($\rm ^{3}He$ ,p           )$\rm ^{6}Li$  & nacr    \\
         $\rm \alpha$  (n            ,$\rm ^{2}H$ )$\rm ^{3}H$   & desc    \\
         $\rm ^{6}Li$  (p            ,$\rm ^{3}He$)$\rm \alpha$  & nacr    \\
         $\rm ^{6}Li$  ($\rm ^{2}H$  ,n           )$\rm ^{7}Be$  & mafo    \\
         $\rm ^{6}Li$  ($\rm ^{2}H$  ,p           )$\rm ^{7}Li$  & mafo    \\
         $\rm ^{6}Li$  (n            ,$\rm ^{3}H$ )$\rm \alpha$  & cf88    \\
         $\rm ^{7}Li$  (p            ,$\rm ^{2}H$ )$\rm ^{6}Li$  & mafo    \\
         $\rm ^{7}Li$  ($\rm ^{2}H$  ,p           )$\rm ^{8}Li$  & mafo    \\
         $\rm ^{7}Li$  ($\rm ^{3}H$  ,n           )$\rm ^{9}Be$  & bb92    \\
         $\rm ^{7}Be$  (n            ,$\rm ^{2}H$ )$\rm ^{6}Li$  & mafo    \\
         $\rm ^{9}Be$  ($\rm ^{3}H$  ,n           )$\rm ^{11}B$  & bb92    \\
         $\rm ^{9}Be$  (n            ,$\rm ^{2}H$ )$\rm ^{8}Li$  & mafo    \\
         $\rm ^{9}Be$  (n            ,$\rm ^{3}H$ )$\rm ^{7}Li$  & bb92    \\
         $\rm ^{11}B$  (n            ,$\rm ^{3}H$ )$\rm ^{9}Be$  & bb92    \\
         $\rm ^{13}C$  ($\rm ^{2}H$  ,n           )$\rm ^{14}N$  & bb92    \\
         $\rm ^{14}C$  ($\rm ^{2}H$  ,n           )$\rm ^{15}N$  & bb92    \\
         $\rm ^{14}N$  (n            ,$\rm ^{2}H$ )$\rm ^{13}C$  & bb92    \\
         $\rm ^{15}N$  (n            ,$\rm ^{2}H$ )$\rm ^{14}C$  & bb92    \\
         $\rm ^{12}C$  ($\rm ^{12}C$ ,n           )$\rm ^{23}Mg$ & da77    \\
         $\rm ^{12}C$  ($\rm ^{12}C$ ,p           )$\rm ^{23}Na$ & cf88    \\
         $\rm ^{12}C$  ($\rm ^{12}C$ ,$\rm \alpha$)$\rm ^{20}Ne$ & cf88    \\
         $\rm ^{12}C$  ($\rm ^{16}O$ ,n           )$\rm ^{27}Si$ & cf88    \\
         $\rm ^{12}C$  ($\rm ^{16}O$ ,p           )$\rm ^{27}Al$ & cf88    \\
         $\rm ^{12}C$  ($\rm ^{16}O$ ,$\rm \alpha$)$\rm ^{24}Mg$ & cf88    \\
         $\rm ^{16}O$  ($\rm ^{16}O$ ,n           )$\rm ^{31}S$  & cf88    \\
         $\rm ^{16}O$  ($\rm ^{16}O$ ,p           )$\rm ^{31}P$  & cf88    \\
         $\rm ^{16}O$  ($\rm ^{16}O$ ,$\rm \alpha$)$\rm ^{28}Si$ & cf88    \\
         $\rm ^{20}Ne$ ($\rm ^{12}C$ ,n           )$\rm ^{31}S$  & rolf    \\
         $\rm ^{20}Ne$ ($\rm ^{12}C$ ,p           )$\rm ^{31}P$  & rolf    \\
         $\rm ^{20}Ne$ ($\rm ^{12}C$ ,$\rm \alpha$)$\rm ^{28}Si$ & rolf    \\
\enddata 
\tablecomments{
cy08 = \citet{cy08};
da77 = \citet{da77};
rolf = C. Rolfs and collaborators;
}
\end{deluxetable*}                                                                                                                                                   
